Duration Dependence and Heterogeneity: Learning from Early Notice of Layoff

This paper presents a novel approach to distinguish the impact of duration-dependent forces and adverse selection on the exit rate from unemployment by leveraging variation in the length of layoff notices. I formulate a Mixed Hazard model in discrete time and specify the conditions under which variation in notice length enables the identification of structural duration dependence while allowing for arbitrary heterogeneity across workers. Utilizing data from the Displaced Worker Supplement (DWS), I employ the Generalized Method of Moments (GMM) to estimate the model. According to the estimates, the decline in the exit rate over the first 48 weeks of unemployment is largely due to the worsening composition of surviving jobseekers. Furthermore, I find that an individual's likelihood of exiting unemployment decreases initially, then increases until unemployment benefits run out, and remains steady thereafter. These findings are consistent with a standard search model where returns to search decline early in the spell.

==> output/tab_ext_notcatA.tex <==
   No notice &   \ensuremath{>}1 month &   1-2 months \\
        0.04 &       0.08 &        -0.01 \\


==> output/tab_ext_notcatB.tex <==
   No notice &   \ensuremath{>}1 month &   1-2 months \\
        0.06 &       0.10 &         0.02 \\

